MOPA: Modular Object Navigation with PointGoal Agents

We propose a simple but effective modular approach MOPA (Modular ObjectNav with PointGoal agents) to systematically investigate the inherent modularity of the object navigation task in Embodied AI. MOPA consists of four modules: (a) an object detection module trained to identify objects from RGB images, (b) a map building module to build a semantic map of the observed objects, (c) an exploration module enabling the agent to explore the environment, and (d) a navigation module to move to identified target objects. We show that we can effectively reuse a pretrained PointGoal agent as the navigation model instead of learning to navigate from scratch, thus saving time and compute. We also compare various exploration strategies for MOPA and find that a simple uniform strategy significantly outperforms more advanced exploration methods.

==> chapters/datasheet.tex <==

\section{DATASHEET: MultiON2.0}
\label{sec:datasheet}

%by Gebru \textit{et al.}
\textbf{This document is based on \textit{Datasheets for Datasets} \cite{gebruDatasheetsDatasets2020}. Please see the most updated version \underline{\textcolor{blue}{\href{http://arxiv.org/abs/1803.09010}{here}}}. }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{mdframed}
\begin{mdframed}[linecolor=\sectioncolor]
\section*{\textcolor{\sectioncolor}{
    MOTIVATION
}}
\end{mdframed}

    \textcolor{\sectioncolor}{\textbf{
    For what purpose was the dataset created?
    }
    %Was there a specific task in mind? Was there
    %a specific gap that needed to be filled? Please provide a description.
    } \\
    %%%
    RxR was created to advance progress on vision-and-language navigation (VLN) in multiple languages (English, Hindi, Telugu). It addresses gaps in existing datasets by including more paths that counter known biases and an order of magnitude more navigation instructions for three languages plus annotators' 3D virtual pose sequences. \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Who created this dataset (e.g., which team, research group) and on behalf
    of which entity (e.g., company, institution, organization)?
    }
    } \\
    %%%
    This dataset was created by Alexander Ku, Peter Anderson, Roma Patel, Eugene Ie, Jason Baldridge and the Google Data Compute team on behalf of Google Research. \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    What support was needed to make this dataset?
    }
    %(e.g.who funded the creation of the dataset? If there is an associated
    %grant, provide the name of the grantor and the grant name and number, or if
    %it was supported by a company or government agency, give those details.)
    } \\
    %%%
    Funding was provided by Google Research. \\
    %%% 
    
    %\textcolor{\sectioncolor}{\textbf{
    %Any other comments?
    %}} \\
    %%%
    %None. \\
    %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mdframed}[linecolor=\sectioncolor]
\section*{\textcolor{\sectioncolor}{
    COMPOSITION
}}
\end{mdframed}
    \textcolor{\sectioncolor}{\textbf{
    What do the instances that comprise the dataset represent (e.g., documents,
    photos, people, countries)?
    }
    %Are there multiple types of instances (e.g., movies, users, and ratings;
    %people and interactions between them; nodes and edges)? Please provide a
    %description.
    } \\
    %%%
     \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    How many instances are there in total (of each type, if appropriate)?
    }
    } \\
    %%%
    \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Does the dataset contain all possible instances or is it a sample (not
    necessarily random) of instances from a larger set?
    }
    %If the dataset is a sample, then what is the larger set? Is the sample
    %representative of the larger set (e.g., geographic coverage)? If so, please
    %describe how this representativeness was validated/verified. If it is not
    %representative of the larger set, please describe why not (e.g., to cover a
    %more diverse range of instances, because instances were withheld or
    %unavailable).
    } \\
    %%%
    \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    What data does each instance consist of?
    }
    %“Raw” data (e.g., unprocessed text or images) or features? In either case,
    %please provide a description.
    } \\
    %%%
    \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Is there a label or target associated with each instance?
    }
    %If so, please provide a description.
    } \\
    %%%
    \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Is any information missing from individual instances?
    }
    %If so, please provide a description, explaining why this information is
    %missing (e.g., because it was unavailable). This does not include
    %intentionally removed information, but might include, e.g., redacted text.
    } \\
    %%%
    \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Are relationships between individual instances made explicit (e.g., users’
    movie ratings, social network links)?
    }
    %If so, please describe how these relationships are made explicit.
    } \\
    %%%
    \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Are there recommended data splits (e.g., training, development/validation,
    testing)?
    }
    %If so, please provide a description of these splits, explaining the
    %rationale behind them.
    } \\
    %%%
    \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Are there any errors, sources of noise, or redundancies in the dataset?
    }
    %If so, please provide a description.
    } \\
    %%%
    \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Is the dataset self-contained, or does it link to or otherwise rely on
    external resources (e.g., websites, tweets, other datasets)?
    }
    %If it links to or relies on external resources, a) are there guarantees
    %that they will exist, and remain constant, over time; b) are there official
    %archival versions of the complete dataset (i.e., including the external
    %resources as they existed at the time the dataset was created); c) are
    %there any restrictions (e.g., licenses, fees) associated with any of the
    %external resources that might apply to a future user? Please provide
    %descriptions of all external resources and any restrictions associated with
    %them, as well as links or other access points, as appropriate.
    } \\
    %%%
    \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Does the dataset contain data that might be considered confidential (e.g.,
    data that is protected by legal privilege or by doctor-patient
    confidentiality, data that includes the content of individuals’ non-public
    communications)?
    }
    %If so, please provide a description.
    } \\
    %%%
     \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Does the dataset contain data that, if viewed directly, might be offensive,
    insulting, threatening, or might otherwise cause anxiety?
    }
    %If so, please describe why.
    } \\
    %%%
    \\
    %%% 
    
    %\textcolor{\sectioncolor}{\textbf{
    %Does the dataset relate to people?
    %}
    %If not, you may skip the remaining questions in this section.
    %} \\
    %%%
    %No. \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Does the dataset identify any subpopulations (e.g., by age, gender)?
    }
    %If so, please describe how these subpopulations are identified and
    %provide a description of their respective distributions within the dataset.
    } \\
    %%%
    No. \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Is it possible to identify individuals (i.e., one or more natural persons),
    either directly or indirectly (i.e., in combination with other data) from
    the dataset?
    }
    %If so, please describe how.
    } \\
    %%%
    \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Does the dataset contain data that might be considered sensitive in any way
    (e.g., data that reveals racial or ethnic origins, sexual orientations,
    religious beliefs, political opinions or union memberships, or locations;
    financial or health data; biometric or genetic data; forms of government
    identification, such as social security numbers; criminal history)?
    }
    %If so, please provide a description.
    } \\
    %%%
    \\
    %%% 
    
    %\textcolor{\sectioncolor}{\textbf{
    %Any other comments?
    %}} \\
    %%%
    %None. \\
    %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mdframed}[linecolor=\sectioncolor]
\section*{\textcolor{\sectioncolor}{
    COLLECTION
}}
\end{mdframed}

    \textcolor{\sectioncolor}{\textbf{
    How was the data associated with each instance acquired?
    }
    %Was the data directly observable (e.g., raw text, movie ratings),
    %reported by subjects (e.g., survey responses), or indirectly
    %inferred/derived from other data (e.g., part-of-speech tags, model-based
    %guesses for age or language)? If data was reported by subjects or
    %indirectly inferred/derived from other data, was the data
    %validated/verified? If so, please describe how.
    } \\
    %%%
    \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Over what timeframe was the data collected?
    }
    %Does this timeframe match the creation timeframe of the data associated
    %with the instances (e.g., recent crawl of old news articles)? If not,
    %please describe the timeframe in which the data associated with the
    %instances was created. Finally, list when the dataset was first published.
    } \\
    %%%
    \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    What mechanisms or procedures were used to collect the data (e.g., hardware
    apparatus or sensor, manual human curation, software program, software
    API)?
    }
    %How were these mechanisms or procedures validated?
    } \\
    %%%
    \\
    %%% 
    
    %\textcolor{\sectioncolor}{\textbf{
    %What was the resource cost of collecting the data?
    %}
    %(e.g. what were the required computational resources, and the associated
    %financial costs, and energy consumption - estimate the carbon footprint.
    %See Strubell \textit{et al.}\cite{strubellEnergyPolicyConsiderations2019} for approaches in this area.)
    %} \\
    %%%
    %\textbf{TODO: cost}. \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    If the dataset is a sample from a larger set, what was the sampling
    strategy (e.g., deterministic, probabilistic with specific sampling
    probabilities)?
    }
    } \\
    %%%
    \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Who was involved in the data collection process (e.g., students,
    crowdworkers, contractors) and how were they compensated (e.g., how much
    were crowdworkers paid)?
    }
    } \\
    %%%
    \\
    %%% 
    
    %\textcolor{\sectioncolor}{\textbf{
    %Were any ethical review processes conducted (e.g., by an institutional
    %review board)?
    %}
    %If so, please provide a description of these review processes, including
    %the outcomes, as well as a link or other access point to any supporting
    %documentation.
    %} \\
    %%%
    %\textbf{TODO..} \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Does the dataset relate to people?
    }
    %If not, you may skip the remainder of the questions in this section.
    } \\
    %%%
    \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Did you collect the data from the individuals in question directly, or
    obtain it via third parties or other sources (e.g., websites)?
    }
    } \\
    %%%
    \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Were the individuals in question notified about the data collection?
    }
    %If so, please describe (or show with screenshots or other information) how
    %notice was provided, and provide a link or other access point to, or
    %otherwise reproduce, the exact language of the notification itself.
    } \\
    %%%
    \\
    %%% 
    
    \textcolor{\sectioncolor}{\textbf{
    Did the individuals in question consent to the collection and use of their
    data?
    }
    %If so, please describe (or show with screenshots or other information) how
    %consent was requested and provided, and provide a link or other access
    %point to, or otherwise reproduce, the exact language to which the
    %individuals consented.
    } \\
    %%%
    \\
    %%% 
    
    %\textcolor{\sectioncolor}{\textbf{
    %If consent was obtained, were the consenting individuals provided with a
    %mechanism to revoke their consent in the future or for certain uses?
    %}
    % If so, please provide a description, as well as a link or other access
    % point to the mechanism (if appropriate)
    %} \\
    %%%
    %No. \\
    %%% 
    
    %\textcolor{\sectioncolor}{\textbf{
    %Has an analysis of the potential impact of the dataset and its use on data
    %subjects (e.g., a data protection impact analysis)been conducted?
    %}
    %If so, please provide a description of this analysis, including the
    %outcomes, as well as a link or other access point to any supporting
    %documentation.
    %} \\
    %%%
    %No. \\
    %%% 
    
    %\textcolor{\sectioncolor}{\textbf{
    %Any other comments?
    %}} \\
    %%%
    %None. \\
    %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mdframed}[linecolor=\sectioncolor]
\section*{\textcolor{\sectioncolor}{PREPROCESSING / CLEANING / LABELING}}
\end{mdframed}

    \textcolor{\sectioncolor}{\textbf{
    Was any preprocessing/cleaning/labeling of the data
    done(e.g.,discretization or bucketing, tokenization, part-of-speech
    tagging, SIFT feature extraction, removal of instances, processing of
    missing values)?
    }
   % If so, please provide a description. If not, you may skip the remainder of
    %the questions in this section.
    } \\
    %%%
    \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Was the “raw” data saved in addition to the preprocessed/cleaned/labeled
    data (e.g., to support unanticipated future uses)?
    }
    %If so, please provide a link or other access point to the “raw” data.
    } \\
    %%%
    \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Is the software used to preprocess/clean/label the instances available?
    }
    %If so, please provide a link or other access point.
    } \\
    %%%
    \\
    %%%

    %\textcolor{\sectioncolor}{\textbf{
    %Any other comments?
    %}} \\
    %%%
    %None. \\
    %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mdframed}[linecolor=\sectioncolor]
\section*{\textcolor{\sectioncolor}{
    USES
}}
\end{mdframed}

    \textcolor{\sectioncolor}{\textbf{
    Has the dataset been used for any tasks already?
    }
    %If so, please provide a description.
    } \\
    %%%
    \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Is there a repository that links to any or all papers or systems that use the dataset?
    }
    %If so, please provide a link or other access point.
    } \\
    %%%
    \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    What (other) tasks could the dataset be used for?
    }
    } \\
    %%%
    \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Is there anything about the composition of the dataset or the way it was
    collected and preprocessed/cleaned/labeled that might impact future uses?
    }
    %For example, is there anything that a future user might need to know to
    %avoid uses that could result in unfair treatment of individuals or groups
    %(e.g., stereotyping, quality of service issues) or other undesirable harms
    %(e.g., financial harms, legal risks) If so, please provide a description.
    %Is there anything a future user could do to mitigate these undesirable
    %harms?
    } \\
    %%%
    \\
    %%%

    %\textcolor{\sectioncolor}{\textbf{
    %Are there tasks for which the dataset should not be used?
    %}
    %If so, please provide a description.
    %} \\
    %%%
    %No. \\
    %%%

    %\textcolor{\sectioncolor}{\textbf{
    %Any other comments?
    %}} \\
    %%%
    %None. \\
    %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mdframed}[linecolor=\sectioncolor]
\section*{\textcolor{\sectioncolor}{
    DISTRIBUTION
}}
\end{mdframed}

    \textcolor{\sectioncolor}{\textbf{
    Will the dataset be distributed to third parties outside of the entity
    (e.g., company, institution, organization) on behalf of which the dataset
    was created?
    }
    %If so, please provide a description.
    } \\
    %%%
    \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    How will the dataset will be distributed (e.g., tarball on website, API,
    GitHub)?
    }
    %Does the dataset have a digital object identifier (DOI)?
    } \\
    %%%
    \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    When will the dataset be distributed?
    }
    } \\
    %%%
    \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Will the dataset be distributed under a copyright or other intellectual
    property (IP) license, and/or under applicable terms of use (ToU)?
    }
    %If so, please describe this license and/or ToU, and provide a link or other
    %access point to, or otherwise reproduce, any relevant licensing terms or
    %ToU, as well as any fees associated with these restrictions.
    } \\
    %%%
    MultiON2.0 is released under a \href{https://creativecommons.org/licenses/by/4.0/}{CC-BY license}. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Have any third parties imposed IP-based or other restrictions on the data
    associated with the instances?
    }
    %If so, please describe these restrictions, and provide a link or other
    %access point to, or otherwise reproduce, any relevant licensing terms, as
    %well as any fees associated with these restrictions.
    } \\
    %%%
    Yes, the Matterport3D dataset is governed by the \href{http://kaldir.vc.in.tum.de/matterport/MP_TOS.pdf}{Matterport3D Terms of Use}. \\
    %%%

    %\textcolor{\sectioncolor}{\textbf{
    %Do any export controls or other regulatory restrictions apply to the
    %dataset or to individual instances?
    %}
    %If so, please describe these restrictions, and provide a link or other
    %access point to, or otherwise reproduce, any supporting documentation.
    %} \\
    %%%
    %No. \\
    %%%

    %\textcolor{\sectioncolor}{\textbf{
    %Any other comments?
    %}} \\
    %%%
    %None. \\
    %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mdframed}[linecolor=\sectioncolor]
\section*{\textcolor{\sectioncolor}{
    MAINTENANCE
}}
\end{mdframed}

    %\textcolor{\sectioncolor}{\textbf{
    %Who is supporting/hosting/maintaining the dataset?
    %}
    %} \\
    %%%
    %The dataset has been released on publication and will be hosted at the GitHub repository here. \textbf{TODO exact link}. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    How can the owner/curator/manager of the dataset be contacted (e.g., email
    address)?
    }
    } \\
    %%%
    \\
    %%%

    %\textcolor{\sectioncolor}{\textbf{
    %Is there an erratum?
    %}
    %If so, please provide a link or other access point.
    %} \\
    %%%
    %No. \\
    %%%

    \textcolor{\sectioncolor}{\textbf{
    Will the dataset be updated (e.g., to correct labeling errors, add new
    instances, delete instances)?
    }
    %If so, please describe how often, by whom, and how updates will be
    %communicated to users (e.g., mailing list, GitHub)?
    } \\
    %%%
    \\
    %%%

    %\textcolor{\sectioncolor}{\textbf{
    %If the dataset relates to people, are there applicable limits on the
    %retention of the data associated with the instances (e.g., were individuals
    %in question told that their data would be retained for a fixed period of
    %time and then deleted)?
    %}
    %If so, please describe these limits and explain how they will be enforced.
    %} \\
    %%%
    %No. \\
    %%%

    %\textcolor{\sectioncolor}{\textbf{
    %Will older versions of the dataset continue to be
    %supported/hosted/maintained?
    %}
    %If so, please describe how. If not, please describe how its obsolescence
    %will be communicated to users.
    %} \\
    %%%
    %N/A. \\
    %%%

    %\textcolor{\sectioncolor}{\textbf{
    %If others want to extend/augment/build on/contribute to the dataset, is
    %there a mechanism for them to do so?
    %}
    %If so, please provide a description. Will these contributions be
    %validated/verified? If so, please describe how. If not, why not? Is there a
    %process for communicating/distributing these contributions to other users?
    %If so, please provide a description.
    %} \\
    %%%
    %Researchers are welcome to augment and extend the dataset as they see fit for certain research directions e.g., more languages for instructions, finer-grained visual annotations and so on. \\
    %%%

    %\textcolor{\sectioncolor}{\textbf{
    %Any other comments?
    %}} \\
    %%%
    %None. \\
    %%%



==> chapters/figures/fig-multion.tex <==
\begin{figure}[t]
    \centering    \includegraphics[width=0.9\linewidth]{img/multion.pdf}
    \caption{Example episode from the \ours task we address.
    % on an HM3D dataset scene. 
    The agent needs to find 5 goals, red, pink, black, blue, and yellow cylinders, in that particular sequence. The rest of the cylinders are distractors.
    % \uj{directionality?}
    }
    \label{fig:multion}
\end{figure}


==> chapters/figures/fig-schematic.tex <==

\begin{figure*}[t]
    \includegraphics[width=\textwidth]{img/schematic.pdf}
    \caption{
    \textbf{Overview.}
    \mon is modular by nature. The agent needs to identify objects from its current view and remember them in a memory (in our case, a map). It needs to explore in order to discover the objects, and once it has seen the current goal, it needs to navigate to it. Our \approach is based on such modularity, consisting of four modules: \objdet, \mapbuilding, \exploration and finally \navigation.
    }
    \label{fig:schematic}
\end{figure*}


==> chapters/figures/fig-teaser-short.tex <==

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{img/teaser_latest.pdf}
\caption{
\textbf{Approach Overview.}
We tackle long-horizon navigation tasks by proposing a modular approach, \approach, to leverage their inherent modularity. Our approach consists of four modules: (1) \textit{\objdet} ($\mathcal{O}$), (2) \textit{\mapbuilding} ($\mathcal{M}$), (3) \textit{\exploration} ($\mathcal{E}$) and (4) \textit{\navigation} ($\mathcal{N}$).
}
\label{fig:teaser_short}
\end{figure}


==> chapters/tables/tab-data-stats-short.tex <==
\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule
        & \multicolumn{2}{c}{Train} & \multicolumn{2}{c}{Validation} & \multicolumn{2}{c}{Test}   \\
        \cmidrule(l{0pt}r{2pt}){2-7}
         & \#Scenes & \#Ep & \#Scenes & \#Ep & \#Scenes & \#Ep   \\ 
         \midrule
        \mon~\cite{wani2020multion} & 61 & 3.05M & 11 & 1050 & 18 & 1050   \\ 
        \ours~(Ours) & 800 & 8.00M & 30 & 1050 & 70 & 1050 \\ 
        \bottomrule
    \end{tabular}}
    \caption{\label{tab-data-stats-short} Dataset comparison of \ours with \mon.
    }
\end{table}


==> chapters/tables/tab-expl-backup.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lllllrrrrrrrr}
    \toprule
        & \multicolumn{4}{c}{\approach Modules}   & \multicolumn{4}{c}{Validation}      & \multicolumn{4}{c}{Test} \\
        \cmidrule(l{0pt}r{2pt}){6-9} \cmidrule(l{2pt}r{0pt}){10-13}
         & $\mathcal{O}$ & $\mathcal{M}$ & $\mathcal{N}$ & $\mathcal{E}$  & Success  & Progress
         & SPL & PPL & Success  & Progress
         & SPL & PPL \\  
        \midrule
        % \orasem & \oracle & \cite{chaplot2020object} &\pointnavshort & \frontier~\cite{yamauchi1997frontier}   &41 \footnotesize{($\pm$ 2)} &50 \footnotesize{($\pm$ 2)} &21 \footnotesize{($\pm$ 1)} &26 \footnotesize{($\pm$ 1)} & 40 \footnotesize{($\pm$ 2)} & 48 \footnotesize{($\pm$ 2)} & 21 \footnotesize{($\pm$ 1)} &25 \footnotesize{($\pm$ 1)} \\ 
        \orasem & \oracle & \cite{chaplot2020object} &\pointnavshort & \stubborn~\cite{luo2022stubborn}    &69 \footnotesize{($\pm$ 2)} &77 \footnotesize{($\pm$ 2)} & 25 \footnotesize{($\pm$ 1)} &27 \footnotesize{($\pm$ 1)} & 66 \footnotesize{($\pm$ 2)} & 75 \footnotesize{($\pm$ 2)} & 23 \footnotesize{($\pm$ 1)} & 26 \footnotesize{($\pm$ 1)}  \\ 
          & & & & \stubbornthresh   &75 \footnotesize{($\pm$ 2)} &82 \footnotesize{($\pm$ 2)} &\textbf{35} \footnotesize{($\pm$ 1)} &\textbf{38} \footnotesize{($\pm$ 1)} & 72 \footnotesize{($\pm$ 2)} & 80 \footnotesize{($\pm$ 2)} & 33 \footnotesize{($\pm$ 1)} & 36 \footnotesize{($\pm$ 1)}  \\
        & & & & \frontier~\cite{yamauchi1997frontier}   &75 \footnotesize{($\pm$ 2)} &81 \footnotesize{($\pm$ 2)} &\textbf{35} \footnotesize{($\pm$ 1)} &37 \footnotesize{($\pm$ 1)} & 72 \footnotesize{($\pm$ 2)} & 80 \footnotesize{($\pm$ 2)} & 33 \footnotesize{($\pm$ 1)} &35 \footnotesize{($\pm$ 1)} \\
        
        & & & & \random  & 78 \footnotesize{($\pm$ 2)} & 84 \footnotesize{($\pm$ 2)} &\textbf{35} \footnotesize{($\pm$ 1)} & 37 \footnotesize{($\pm$ 1)} & 72 \footnotesize{($\pm$ 2)}  & 80 \footnotesize{($\pm$ 2)}  & 33 \footnotesize{($\pm$ 1)} & 36 \footnotesize{($\pm$ 1)}  \\ 
        
        & & & & \newadd{\ansglobal}\cite{chaplot2020learning} & 78 \footnotesize{($\pm$ 2)} & 84 \footnotesize{($\pm$ 2)} &\textbf{35} \footnotesize{($\pm$ 1)} & 37 \footnotesize{($\pm$ 1)} &76 \footnotesize{($\pm$ 2)} & 83 \footnotesize{($\pm$ 2)} & 35 \footnotesize{($\pm$ 1)} &38 \footnotesize{($\pm$ 1)}  \\
        
        & & & & \randthresh   & \textbf{80} \footnotesize{($\pm$ 2)} & \textbf{87} \footnotesize{($\pm$ 2)} & \textbf{35} \footnotesize{($\pm$ 1)} &\textbf{38} \footnotesize{($\pm$ 1)}  & \textbf{81} \footnotesize{($\pm$ 2)}  & \textbf{87} \footnotesize{($\pm$ 2)}  & \textbf{37} \footnotesize{($\pm$ 1)} & \textbf{39} \footnotesize{($\pm$ 1)}   \\
          
    \bottomrule
    \end{tabular}}
    \caption{
    \textbf{Study of the \exploration module.}
    We find that the simple \randthresh outperforms Stubborn and Frontier-based exploration in \approach.
    We study the contribution of the \exploration ($\mathcal{E}$) module by fixing the other modules to use ground truth (`\oracle') semantic labels in the \objdet ($\mathcal{O}$) module, \mapbuilding ($\mathcal{M}$) from \cite{chaplot2020object} and \pointnav (`\pointnavshort') as the \navigation ($\mathcal{N}$) module.
    }
    \label{tab:exploration_exp}
\end{table*}

==> chapters/tables/tab-main-exp-short.tex <==
\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lllrrrr}
    \toprule
        & Dataset & \objdet   & \multicolumn{4}{c}{Val} \\
        \cmidrule(l{0pt}r{2pt}){4-7} 
        & & & Success  & Progress
         & SPL & PPL \\ 
        \midrule
        \predsem & \ours(CYL) & \frcnnshort\cite{ren2015faster} &50  &65  &21  &26  \\
        
         & \ours(NAT) & \frcnnshort\cite{ren2015faster} & 28  &47  &11  &18   \\
        
        & ObjNav-2022\cite{habitatchallenge2022}  & RedNet\cite{jiang2018rednet, cartillier2020semantic}   &30 &- &28 &-  \\
        
        % \cmidrule(l{0pt}r{2pt}){2-11}
        \midrule
        
        \orasem & \ours(CYL) &  \oracle  & 80  & 87  & 35  &38  \\

         & \ours(NAT) & \oracle   & 80  &85  &35  &38  \\

         & ObjNav-2022\cite{habitatchallenge2022} & \oracle   &64 &- &30 &-  \\
        
    \bottomrule
    \end{tabular}}
    \caption{
    \textbf{\approach performance.} \orasem, using oracle semantic labels, outperforms \predsem in general. \predsem performs better on Cylinder objects than Natural objects in MultiON, and considerably well on the ObjectNav task. These experiments use \random as \exploration ($\mathcal{E}$), \pointnav~\cite{ramakrishnan2021hm3d} (`\pointnavshort') as \navigation ($\mathcal{N}$) and \cite{chaplot2020object} as \mapbuilding ($\mathcal{M}$).
    }
    \label{tab:main_results_short}
\end{table}

==> chapters/tables/tab-nav-backup.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lllllrrrrrrrr}
    \toprule
        & \multicolumn{4}{c}{\approach Modules}  & \multicolumn{4}{c}{Validation}      & \multicolumn{4}{c}{Test} \\
        \cmidrule(l{0pt}r{2pt}){6-9} \cmidrule(l{2pt}r{0pt}){10-13}
         & $\mathcal{O}$ & $\mathcal{M}$  & $\mathcal{E}$ & $\mathcal{N}$ & Success  & Progress
         & SPL & PPL & Success  & Progress
         & SPL & PPL \\  
        \midrule
        \orasem   &  \oracle & \cite{chaplot2020object} & \randthreshshort &\fastmarching\cite{chaplot2020learning}  &19 \footnotesize{($\pm$ 2)} &37 \footnotesize{($\pm$ 2)} &13 \footnotesize{($\pm$ 1)} &25 \footnotesize{($\pm$ 1)} &18 \footnotesize{($\pm$ 2)} & 36 \footnotesize{($\pm$ 2)} &11 \footnotesize{($\pm$ 1)} & 21 \footnotesize{($\pm$ 1)}\\
         & && &\bfs~\cite{deitke2022retrospectives} & 27 \footnotesize{($\pm$ 2)} & 41 \footnotesize{($\pm$ 2)} & 19 \footnotesize{($\pm$ 1)} & 29 \footnotesize{($\pm$ 1)} & 21 \footnotesize{($\pm$ 2)} & 44 \footnotesize{($\pm$ 2)} & 12 \footnotesize{($\pm$ 1)} & 22 \footnotesize{($\pm$ 1)} \\
         
         % & && &\shortest*\cite{savva2019habitat} &74 \footnotesize{($\pm$ 2)} &82 \footnotesize{($\pm$ 2)} &\textbf{39} \footnotesize{($\pm$ 1)} &\textbf{43} \footnotesize{($\pm$ 1)} &71 \footnotesize{($\pm$ 2)} &79 \footnotesize{($\pm$ 2)} &37 \footnotesize{($\pm$ 1)} &\textbf{42} \footnotesize{($\pm$ 1)}\\
         % & && &\newadd{\shortestimp}* &75 \footnotesize{($\pm$ 2)} &84 \footnotesize{($\pm$ 2)} &\textbf{39} \footnotesize{($\pm$ 1)}  &\textbf{43} \footnotesize{($\pm$ 1)}  &76 \footnotesize{($\pm$ 2)} &83 \footnotesize{($\pm$ 2)} &\textbf{39} \footnotesize{($\pm$ 1)} &\textbf{42} \footnotesize{($\pm$ 1)}\\

        & && &\newadd{\shortest}* &75 \footnotesize{($\pm$ 2)} &84 \footnotesize{($\pm$ 2)} &\textbf{39} \footnotesize{($\pm$ 1)}  &\textbf{43} \footnotesize{($\pm$ 1)}  &76 \footnotesize{($\pm$ 2)} &83 \footnotesize{($\pm$ 2)} &\textbf{39} \footnotesize{($\pm$ 1)} &\textbf{42} \footnotesize{($\pm$ 1)}\\
         
        &  & & &       \pointnav~\cite{ramakrishnan2021hm3d}  & \textbf{80} \footnotesize{($\pm$ 2)} & \textbf{87} \footnotesize{($\pm$ 2)} & 35 \footnotesize{($\pm$ 1)} &38 \footnotesize{($\pm$ 1)}  & \textbf{81} \footnotesize{($\pm$ 2)}  & \textbf{87} \footnotesize{($\pm$ 2)}  & 37 \footnotesize{($\pm$ 1)} & 39 \footnotesize{($\pm$ 1)} \\
         
    \bottomrule
    \end{tabular}}
    \caption{
    \textbf{Study of the \navigation module.}
    We observe that a learned \pointnav, when used as the \navigation ($\mathcal{N}$) module in \approach, outperforms analytical path planners (\bfsshort, \shortest \& \fastmarchingshort) on Success and Progress. Note that the \shortest plans the shortest path to the goal based on the ground truth navigation meshes 
    % from the Habitat simulator 
    which accounts for its high SPL and PPL. In these experiments, we fix other modules to use ground truth (`\oracle') semantic labels in the \objdet ($\mathcal{O}$) module, \mapbuilding ($\mathcal{M}$) from \cite{chaplot2020object} and \randthresh (`\randthreshshort') as the \exploration ($\mathcal{E}$) module. 
    % We employ the best-performing \randthresh across these baselines. 
    % \textbf{Quantitative results (navigation policies).}
    % We find that the analytical \bfs path-planner performs considerably worse than the learned \pointnav on the 3ON (cylinders) task.
    % (2) \pointnav (~12hrs) is ~4times faster than BFS  path planner (~48hrs). 
    % Above set of experiments are on 3ON cylinders test set with the best performing exploration strategy from \cref{tab:exploration_exp}, i.e., \randthresh.
    % \uj{oracle choices for OD weakens this}
    % \uj{re-order to have increasing performance from top to bottom}
    }
    \label{tab:nav_exp}
\end{table*}

==> chapters/tables/tab-objnav-hm3d-full.tex <==
\begin{table}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}lllllrrr@{}}
    \toprule
         % \multirow{2}{*}{ObjectNav} 
         &\multirow{2}{*}{Method} &\multirow{2}{*}{\thead[l]{Object\\ Detection}} &\multirow{2}{*}{Exploration} &\multirow{2}{*}{Navigation} & \multicolumn{2}{c}{Validation}  \\
        \cmidrule(l{0pt}r{2pt}){6-7}
        & &&  & & Success   & SPL \\ 
        \midrule
        
        %HM3D~\cite{habitatchallenge2022} 
        &\orasem  &\oracle &\randthreshshort &\pointnavshort &64 &32 \\

        &\orasem  &\oracle &SemExp\cite{chaplot2020object} &\pointnavshort & 60 & 30 \\

        \cmidrule(l{0pt}r{2pt}){2-7}

         &\predsem &Detic\cite{zhou2022detecting}  &\randthreshshort &\pointnavshort &30 &14 \\

         & &Detic\cite{zhou2022detecting}  & SemExp\cite{chaplot2020object} &\pointnavshort & 25 &12  \\

        & &Mask-RCNN\cite{he2017mask}  &\randthreshshort &\pointnavshort &19 &10 \\
        & &Mask-RCNN\cite{he2017mask} & SemExp\cite{chaplot2020object} &\pointnavshort &16 &8  \\
        & &Mask-RCNN\cite{he2017mask} & SemExp\cite{chaplot2020object} &\fastmarchingshort &15 &6 \\

        \cmidrule(l{0pt}r{2pt}){2-7}

        &ModLearn\cite{gervet2023navigating} &\oracle &SemExp\cite{chaplot2020object} &\fastmarchingshort &62 &32 \\

        & &Detic\cite{zhou2022detecting} &SemExp\cite{chaplot2020object} &\fastmarchingshort &27 & 16 \\
        
        & &Mask-RCNN\cite{he2017mask} &SemExp\cite{chaplot2020object} &\fastmarchingshort &29 &17 \\
        

        % \cmidrule(l{0pt}r{2pt}){2-7}
        % & ZSON\cite{majumdar2022zson} & CLIP\cite{radford2021learning} &&  &25 & 13 \\
        
    \bottomrule
        \end{tabular}}
    \caption{\textbf{ObjectNav performance on Habitat ObjectNav 2022 challenge dataset.} 
    % \orasem agent, which uses ground-truth semantic labels, performs similarly on both versions of ObjectNav.
   Using the Detic detector outperforms Mask-RCNN. 
    % on both datasets.
    %Detic achieves slightly better success than RedNet in our \predsem agent. 
    }
    \label{tab:momon_objnav_hm3d_full}
\end{table}

==> chapters/tables/tab-old.tex <==





% \begin{table}[!ht]
%     \centering
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{|l|cc|cc|cc|cc|}
%     \hline
%         & \multicolumn{2}{c|}{Success (\%)}                       & \multicolumn{2}{c|}{Progress (\%)} 
%          & \multicolumn{2}{c|}{SPL (\%)} 
%           & \multicolumn{2}{c|}{PPL (\%)} \\ 
%         \cline{2-9}
%         Baselines & CYL & REAL & CYL & REAL & CYL & REAL & CYL & REAL  \\ 
%          \hline
%         GRU(DD-PPO)~\cite{wijmans2019dd} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ 
%         ProjNeuralMap & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~   \\ 
%         ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~  \\ \hline
%     \end{tabular}}
%     \caption{Baseline Results on CYL and REAL tracks: method x does better than method y.}
% \end{table}


% \subsection{3ON vs 3ON2.0}
% \begin{table}[!ht]
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
%                 & Success & Progress & PPL   & SPL  & DTS  \\ \hline
% 3ON1.0 Test set & 9       & 27       & 10.44 & 4.68 & 5.57 \\ \hline
% 3ON2.0 Test set & 0.1     & 5.56     & 1.77  & 0.07 & 8.16 \\ \hline
% \end{tabular}
%     \caption{Pretrained model on 3ON1.0 applied to 3ON1.0 and 3ON2.0 test sets.}
% \end{table}

% \begin{table}[!ht]
%     \begin{tabular}{|l|l|l|l|l|}
%     \hline
%             & Progress  & PPL    & Success & SPL    \\ \hline
%         1ON & 0.2543    & 0.1541 & 0.2543  & 0.1541 \\ \hline
%         2ON & 0.1914    & 0.0859 & 0.0714  & 0.0378 \\ \hline
%         3ON & 0.1254    & 0.0546 & 0.0200  & 0.0107 \\ \hline
%         4ON & 0.0864    & 0.0387 & 0.0010  & 0.0004 \\ \hline
%         5ON & 0.0720    & 0.0327 & 0.0010  & 0.0004 \\ \hline
%     \end{tabular}
%     \caption{Fixed number of distractors, variable number of goals. (proj-neural agent)}
% \end{table}


==> chapters/tables/tab-sem-map-exp.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{llllllcccccccc}
    \toprule
        & \multicolumn{4}{c}{\approach} & Objects  & \multicolumn{4}{c}{Validation}      & \multicolumn{4}{c}{Test} \\
        \cmidrule(l{0pt}r{2pt}){7-10} \cmidrule(l{2pt}r{0pt}){11-14}
          & \mapbuildingshort  & \explorationshort & \navigationshort & \objdetshort & & Success  & Progress
         & SPL & PPL & Success  & Progress
         & SPL & PPL \\
        \midrule
        \orasem & M & \randthreshshort & \pointnavshort & \oracle & CYL & 80 ($\pm$ 2) & 87 ($\pm$ 2) & 35 ($\pm$ 1) &38 ($\pm$ 1)  & 81 ($\pm$ 2)  & 87 ($\pm$ 2)  & 37 ($\pm$ 1) & 39 ($\pm$ 1)\\ 
        \predsem &  & & & FasterRCNN+KNN & &50 ($\pm$ 2) &65 ($\pm$ 2) &21 ($\pm$ 1) &26 ($\pm$ 1) &52 ($\pm$ 2) &66 ($\pm$ 2) &21 ($\pm$ 1) &27 ($\pm$ 1) \\
        
        \cmidrule(l{0pt}r{2pt}){2-14}
        
        \orasem & M & \randthreshshort & \pointnavshort & \oracle & NAT & 80 ($\pm$ 2) &85 ($\pm$ 2) &35 ($\pm$ 1) &38 ($\pm$ 1) &81 ($\pm$ 2) &87 ($\pm$ 2) &37 ($\pm$ 1) &39 ($\pm$ 1)\\ 
        \predsem &  & & & FasterRCNN &  & 28 ($\pm$ 2) &47 ($\pm$ 2) &11 ($\pm$ 1) &18 ($\pm$ 1) &29 ($\pm$ 2) &45 ($\pm$ 2) &11 ($\pm$ 1) &17 ($\pm$ 1) \\
    \bottomrule
    \end{tabular}}
    \caption{
    \textbf{\objdet module performance.}
    % \textbf{Quantitative results (\orasem \& \predsem).} 
    %\todo{what inference to draw here?}
    We replace the \oracle semantic labels in the \objdet module with a learned object detector and see a drop in the performance of the \approach. Furthermore, we notice that the performance for NAT objects are worse than the CYL objects indicating that the NAT objects are harder to detect.
    % The \predsem agent performs significantly worse than the \orasem agent, due to error in the Object Detector.
    The above set of experiments are on 3ON folds using the \mapbuilding from \cite{chaplot2020object} (M), \randthresh (\randthreshshort) as the \exploration module and \pointnav (\pointnavshort) as the \navigation module.
    % using the best-performing modules for \navigation (\pointnav) and \exploration (\randthresh).
    % \todo{We will use RedNET to improve the \predsem agent for both CYL and NAT}
    }
    \label{tab:sem_map_exp}
\end{table*}

==> chapters/task.tex <==
In the MultiON task \cite{wani2020multion}, is required for an agent to search and approach a fixed sequence of \textit{N} cylinders (each of them with a different color) in an unexplored environment. The cylinders were spawned in navigable locations and are not collidable.
The agent is equipped with an RGB-D sensor that gives 2D images of the current view and with a GPS+Compass sensor, which gives the current coordinates relatively to the starting point. So the agent can use as inputs the RGB-D image, the coordinates of its current position, and the next goal to be found.
The agent starts from a random location inside the environment and has $2500$ actions (called steps) to find all the requested objects in the given order. The action space comprises four possibilities: (i) \textbf{MOVE\_FORWARD} by 25 cm; (ii) \textbf{TURN\_LEFT} by 30°; (iii) \textbf{TURN\_RIGHT} by 30°; (iv) \textbf{FOUND}. The FOUND action, when enabled, has two distinct behaviour: if the agent is below a certain threshold $d$ (set to one meter) from the current object goal, the action succeeds and the agent continues its exploration, otherwise, if the agent is farther then $d$, the episode fails.
In particular, the sequence has a fixed length, and the agent at each step only knows the next object to find. Once found, it will then be notified of the next one, and so on until the task is completed. In \cite{wani2020multion}, the authors explored and constructed the 1ON, 2ON and 3ON tasks. We modified the original setup, by introducing other two object goals (5ON task). Furthermore, while in the original setup only the goal objects were placed inside the environment, we also added some distractor objects. These distractors are always cylinders, but not required for the current episode. We kept the same cylinders from \cite{wani2020multion}, for a total of 8 different objects. Summing up, each episode in our reformulation contains five object goals and distractors. 

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{img/REAL_OBJS_MULTION.png}
    \caption{}
    \label{fig:REAL_OBJS}
\end{figure}

